An Advanced Tree Algorithm with Interference Cancellation in Uplink and Downlink

In this paper, we propose Advanced Tree-algorithm with Interference Cancellation (ATIC), a variant of binary tree-algorithm with successive interference cancellation (SICTA) introduced by Yu and Giannakis. ATIC assumes that Interference Cancellation (IC) can be performed both by the access point (AP), as in SICTA, but also by the users. Specifically, after every collision slot, the AP broadcasts the observed collision as feedback. Users who participated in the collision then attempt to perform IC by subtracting their transmissions from the collision signal. This way, the users can resolve collisions of degree 2 and, using a simple distributed arbitration algorithm based on user IDs, ensure that the next slot will contain just a single transmission. We show that ATIC reaches the asymptotic throughput of 0.924 as the number of initially collided users tends to infinity and reduces the number of collisions and packet delay. We also compare ATIC with other tree algorithms and indicate the extra feedback resources it requires.

==> tables/MSTCompare.tex <==
\setlength\tabcolsep{1pt}
\begin{table}
\centering
    \resizebox{0.5\columnwidth}{!}
    {%
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Algorithm & MST & Access \\
    \hline
    \ac{STA}&  0.429&  Windowed\\
    \hline
    MTA & 0.488 & Windowed\\
    \hline
    SICTA & 0.692 & Blocked\\
    \hline
    ATIC & 0.924 &Blocked\\
    \hline
    \end{tabular}}
    \caption{Summary of the MST for different tree algorithms, rounded to 3 significant figures.}
    \label{tab:summary}
\end{table}

==> tables/memorytable.tex <==
%\setlength\tabcolsep{1pt}
\begin{table}[h]
    %\resizebox{\columnwidth}{!}
    {%
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Slot &AP & User 1 & User 2 & User 3 & User 4\\
    \hline
    0&  & $A$ & $B$ & $C$ & $D$\\
    \hline
    1& $A+B+C+D$ & $A$, $B+C+D$ & $B$, $A+C+D$ & $C$, $A+B+D$ & $D$, $A+B+C$\\
    \hline
    2&$A+B+C$, $D$ & $A$, $B+C$ & $B$, $A+C$ & $C$, $A+B$ & $D$, $A+B+C$\\
    \hline
    3&$A+B$, $C$, $D$ & $A$, $B$ & $B$, $A$ & $C$, $A+B+D$ & $D$, $A+B+C$\\
    \hline
    4&$A$, $B$, $C$, $D$ & $A$, $B$ & $B$, $A$ & $C$, $A+B+D$ & $D$, $A+B+C$\\
    \hline
    \end{tabular}}
    \caption{Listing the memory for the access point and each user, see also Figure \ref{fig:tree_example}.}
    \label{tab:result_table}
\end{table}

